AdaCM$^2$: On Understanding Extremely Long-Term Video with Adaptive Cross-Modality Memory Reduction

The advancements in large language models (LLMs) have propelled the improvement of video understanding tasks by incorporating LLMs with visual models. However, most existing LLM-based models (e.g., VideoLLaMA, VideoChat) are constrained to processing short-duration videos. Recent attempts to understand long-term videos by extracting and compressing visual features into a fixed memory size. Nevertheless, those methods leverage only visual modality to merge video tokens and overlook the correlation between visual and textual queries, leading to difficulties in effectively handling complex question-answering tasks. To address the challenges of long videos and complex prompts, we propose AdaCM$^2$, which, for the first time, introduces an adaptive cross-modality memory reduction approach to video-text alignment in an auto-regressive manner on video streams. Our extensive experiments on various video understanding tasks, such as video captioning, video question answering, and video classification, demonstrate that AdaCM$^2$ achieves state-of-the-art performance across multiple datasets while significantly reducing memory usage. Notably, it achieves a 4.5% improvement across multiple tasks in the LVU dataset with a GPU memory consumption reduction of up to 65%.

==> tables/table6.tex <==
% \renewcommand{\arraystretch}{0.95}
% \begin{tabular}{>{\raggedright\arraybackslash}p{0.6cm}>{\raggedright\arraybackslash}p{0.6cm}|>{\raggedright\arraybackslash}p{1.2cm}>{\raggedright\arraybackslash}p{1cm}>{\raggedright\arraybackslash}p{1cm}|>{\raggedright\arraybackslash}p{1.1cm}}
% \begin{tabular}{>{\raggedright\arraybackslash}p{0.6cm}>{\raggedright\arraybackslash}p{0.6cm}|>{\raggedright\arraybackslash}p{1.2cm}>{\raggedright\arraybackslash}p{1cm}|>{\raggedright\arraybackslash}p{1.1cm}}
%     \toprule
%      $\beta$ & $\alpha$ & \textbf{MSRVTT} & \textbf{MSVD}& \textbf{Mem(GB)} \\
%     \midrule
%     \rowcolor{blue!12}
%     0.1 & 0.1 & {44.92}  & {59.15} & 16.957 \\
%     \midrule
%      0.2$\uparrow$ & 0.1 & 45.26\textcolor{green}{$\uparrow$} & 59.56\textcolor{green}{$\uparrow$}  & 16.961\\
%       0.3$\uparrow$ & 0.1 & 44.87\textcolor{red}{$\downarrow$} & 59.30\textcolor{green}{$\uparrow$} &  16.967\\
%       0.4$\uparrow$ & 0.1 & 46.20\textcolor{green}{$\uparrow$}& 59.10\textcolor{red}{$\downarrow$} &  16.975\\
%       0.5$\uparrow$ & 0.1 & 46.45\textcolor{green}{$\uparrow$} & 58.93\textcolor{red}{$\downarrow$} &  16.996\\
%       0.6$\uparrow$ & 0.1 & 46.07\textcolor{green}{$\uparrow$} & 58.87\textcolor{red}{$\downarrow$} &  17.014 \\
%       0.7$\uparrow$ & 0.1 & 44.35\textcolor{red}{$\downarrow$} & 58.93 & 17.050 \\
%       % 0.8$\uparrow$ & 0.1 & 44.41 & 59.42 & - \\
%       % 0.9$\uparrow$ & 0.1 & 44.86 & 59.29 & -\\
%       \midrule
%       0.1 & 0.2$\uparrow$ & 45.16\textcolor{green}{$\uparrow$}  & 59.31\textcolor{green}{$\uparrow$} &  16.961 \\
%       0.1 & 0.3$\uparrow$ & 44.79\textcolor{red}{$\downarrow$}  & 59.42\textcolor{green}{$\uparrow$} &  16.967 \\
%       0.1 & 0.4$\uparrow$ & 46.09\textcolor{green}{$\uparrow$}  & 59.19\textcolor{green}{$\uparrow$} &  16.975 \\
%       0.1 & 0.5$\uparrow$ & 46.39\textcolor{green}{$\uparrow$}  & 59.03\textcolor{red}{$\downarrow$} &  16.996 \\
%       0.1 & 0.6$\uparrow$ & 45.94\textcolor{green}{$\uparrow$}  & 58.85\textcolor{red}{$\downarrow$} &  17.014 \\
%       0.1 & 0.7$\uparrow$ & 44.330\textcolor{red}{$\downarrow$}  & 59.04\textcolor{red}{$\downarrow$} &  17.050 \\
%       % 0.1 & 0.8$\uparrow$ & 44.336\textcolor{red}{$\downarrow$}  & 59.18 & - \\
%       % 0.1 & 0.9$\uparrow$ & 44.255\textcolor{red}{$\downarrow$}  & 59.22 & - \\
%       % \midrule
%       %  0.2 & 0.2$\uparrow$ & 44.83\textcolor{red}{$\downarrow$} & 59.38\textcolor{green}{$\uparrow$} & 50.29\textcolor{red}{$\downarrow$} & 16.967\\
%       %  0.2 & 0.3$\uparrow$ & 46.16\textcolor{green}{$\uparrow$} & 59.14\textcolor{red}{$\downarrow$} & 50.40\textcolor{red}{$\downarrow$} & 16.975\\
%     \bottomrule
% \end{tabular}


